Forking: Sudden Overfitting Under Replay

This paper studies forking, a generalization failure discovered in NanoGPT autoresearch. Under data replay, models with an over-encoding n-gram memory branch show a sharp separation of training and validation loss at epoch boundaries, resembling the shape of forks. We study this phenomenon in a controlled vanilla NanoGPT setting and reproduce it in a DeepSeek-style model with Engram. Mechanistically, repeated updates sharpen the continuations observed in training while suppressing the probability of unseen continuations, whose loss grows with each pass. The n-gram module creates weakly interacting context-specific subspaces, amplifying this effect. Low-frequency contexts contribute most of the gap, whereas larger training budgets and heavily crowded tables suppress it. We also observe forking in short-budget, heavily repeated SFT and RL-like regimes. The contributions of this paper are twofold: (1) Forking reveals yet another curious phenomenon in deep learning, in addition to grokking and double descent. (2) Forking is an unexpected and unpleasant by-product of tricks proposed by autoresearch agents. While these agents produce an enormous number of results that seem useful, we should always be careful with their results.

==> tables/parameter_selection_initial.tex <==
% Generated by build_evidence.py; raw logged records.
\begin{tabular}{rrrrr}
\toprule
$\eta_B^{\max}$ & $\eta_T^{\max}$ & Train & Validation & Gap \\
\midrule
0.0004 & 0.0008 & 3.121 & 4.309 & 1.187 \\
0.0006 & 0.0012 & 2.899 & 4.433 & 1.534 \\
0.004 & 0.008 & 6.174 & 6.234 & 0.060 \\
\bottomrule
\end{tabular}


==> tables/parameter_selection_locked.tex <==
% Generated by build_evidence.py; raw logged records.
\begin{tabular}{rrrrrr}
\toprule
$\eta_B^{\max}$ & Train & Validation & Input gap & No-gram gap & Net gap \\
\midrule
0.00006 & 2.475 & 5.522 & 3.047 & 0.057 & 2.991 \\
0.0001 & 2.151 & 5.733 & 3.582 & 0.073 & 3.508 \\
0.0003 & 1.545 & 6.411 & 4.866 & 0.163 & 4.702 \\
0.0006 & 1.251 & 6.940 & 5.689 & 0.255 & 5.434 \\
0.001 & 1.243 & 7.269 & 6.026 & 0.195 & 5.831 \\
0.002 & 1.487 & 7.332 & 5.844 & 0.075 & 5.770 \\
0.004 & 6.694 & 6.741 & 0.046 & 0.014 & 0.032 \\
\bottomrule
\end{tabular}


==> tables/parameter_selection_scale.tex <==
% Generated by build_evidence.py; raw logged records.
\begin{tabular}{rrrrrr}
\toprule
$s_T$ & $\eta_T^{\max}$ & Train$_{1000}$ & Validation$_{1000}$ & $G_{1000}$ & $G_{2000}$ \\
\midrule
0.5 & 0.0003 & 3.521 & 3.986 & 0.465 & -- \\
1 & 0.0006 & 3.265 & 4.123 & 0.858 & -- \\
2 & 0.0012 & 2.883 & 4.433 & 1.551 & -- \\
3 & 0.0018 & 2.759 & 4.645 & 1.886 & -- \\
4 & 0.0024 & 2.757 & 4.830 & 2.072 & -- \\
8 & 0.0048 & 2.652 & 5.080 & 2.428 & 6.020 \\
16 & 0.0096 & 2.689 & 5.328 & 2.639 & 5.761 \\
32 & 0.0192 & 2.637 & 5.284 & 2.647 & 5.659 \\
64 & 0.0384 & 2.572 & 5.278 & 2.706 & 5.740 \\
128 & 0.0768 & 2.547 & 5.279 & 2.732 & 5.724 \\
256 & 0.1536 & 2.621 & 5.299 & 2.677 & 5.543 \\
512 & 0.3072 & 2.669 & 5.240 & 2.571 & 5.474 \\
1024 & 0.6144 & 2.805 & 5.255 & 2.450 & 5.335 \\
\bottomrule
\end{tabular}

